Moral Machine or Tyranny of the Majority?

With Artificial Intelligence systems increasingly applied in consequential domains, researchers have begun to ask how these systems ought to act in ethically charged situations where even humans lack consensus. In the Moral Machine project, researchers crowdsourced answers to "Trolley Problems" concerning autonomous vehicles. Subsequently, Noothigattu et al. (2018) proposed inferring linear functions that approximate each individual's preferences and aggregating these linear models by averaging parameters across the population. In this paper, we examine this averaging mechanism, focusing on fairness concerns in the presence of strategic effects. We investigate a simple setting where the population consists of two groups, with the minority constituting an {\alpha} < 0.5 share of the population. To simplify the analysis, we consider the extreme case in which within-group preferences are homogeneous. Focusing on the fraction of contested cases where the minority group prevails, we make the following observations: (a) even when all parties report their preferences truthfully, the fraction of disputes where the minority prevails is less than proportionate in {\alpha}; (b) the degree of sub-proportionality grows more severe as the level of disagreement between the groups increases; (c) when parties report preferences strategically, pure strategy equilibria do not always exist; and (d) whenever a pure strategy equilibrium exists, the majority group prevails 100% of the time. These findings raise concerns about stability and fairness of preference vector averaging as a mechanism for aggregating diverging voices. Finally, we discuss alternatives, including randomized dictatorship and median-based mechanisms.

==> sections/conclusion.tex <==
\mfcomment{TODO REVISE}

In conclusion, we have provided detailed analysis of how the averaging aggregation mechanism outlined in \citet{noothigattu2018voting} has several characteristics that may be unwanted. Specifically, it is susceptible to manipulation and tyranny of the majority, and even when voters report their true preferences, concessions to the minority group are sublinear. \mfedit{Alternatives to this averaging mechanism exist, including but not limited to aggregation via medians and randomized dictatorship, that ameliorate some of these drawbacks, but they in turn have pitfalls of their own.} We hope that our insights can effectively aid machine learning practitioners in rethinking their aggregation schemes and participation mechanisms as a whole when building \mfedit{crowdsourced decision-making  algorithms.}
